Unstable recurrent patterns in Kuramoto-Sivashinsky dynamics

We undertake a systematic exploration of recurrent patterns in a 1-dimensional Kuramoto-Sivashinsky system. For a small, but already rather turbulent system, the long-time dynamics takes place on a low-dimensional invariant manifold. A set of equilibria offers a coarse geometrical partition of this manifold. A variational method enables us to determine numerically a large number of unstable spatiotemporally periodic solutions. The attracting set appears surprisingly thin - its backbone are several Smale horseshoe repellers, well approximated by intrinsic local 1-dimensional return maps, each with an approximate symbolic dynamics. The dynamics appears decomposable into chaotic dynamics within such local repellers, interspersed by rapid jumps between them.

==> acknow.tex <==
% acknow.tex
%
% Lan                                           ??jul2004
% Predrag                                       23jul2004


\Preliminary{
        \begin{acknowledgments}

We would like to thank ?? for careful reading of the
manuscript and numerous suggestions, and
?? for bringing refrefs?? %{fl92,tompaid96}
to our attention.

        \end{acknowledgments}
        } %end \preliminary{




==> type.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% draft version
% Predrag			mar 20 2006
% script ./update copies this into type.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \newif\ifdraft
		% comment out the undesired features (one of 2): 
\drafttrue	% editing version:
		%   includes margin comments, \Preliminary{...} parts
%\draftfalse	% public version:
		%   omits    margin comments, \Preliminary{...} parts

%%%%%%%%%%%%%%%%%%%%%% PS or PDF? %%%%%%%%%%%%%%%%%%%
%
\newif\ifpdf 
		% comment out the undesired features (one of 2): 
\pdffalse 	% prepare dvi file for dvips -> PostScript
%\pdftrue 	% prepare dvi file for Acrobat Destiller -> HyperTeX pdf 

%%%%%%%%%%%%%%%%%% REMEMBER:
                %% generate 
		%% > bibtex ks  
		%% then execute again
		%% > latex ks

